An Eigenshapes Approach to Compressed Signed Distance Fields and Their Utility in Robot Mapping

In order to deal with the scaling problem of volumetric map representations we propose spatially local methods for high-ratio compression of 3D maps, represented as truncated signed distance fields. We show that these compressed maps can be used as meaningful descriptors for selective decompression in scenarios relevant to robotic applications. As compression methods, we compare using PCA-derived low-dimensional bases to non-linear auto-encoder networks and novel mixed architectures that combine both. Selecting two application-oriented performance metrics, we evaluate the impact of different compression rates on reconstruction fidelity as well as to the task of map-aided ego-motion estimation. It is demonstrated that lossily compressed distance fields used as cost functions for ego-motion estimation, can outperform their uncompressed counterparts in challenging scenarios from standard RGB-D data-sets.

==> table.tex <==
\begin{table*}[ht]
\begin{centering}
    \begin{tabular}{|l|c|c|c|c|c|}
    \hline
    Reconstruction Method   & Reconstruction Error (MSE)$\pm\sigma$ & Mean ATE [m] $\pm\sigma$          & Median ATE [m] & Mean RPE [m] $\pm\sigma$ & Median RPE [m] \\ \hline
    Original data           & -                                     & 0.70$\pm$ 0.67                    & 0.59           &  0.024$\pm$\textbf{0.041}          & 0.012          \\ \hline
    PCA 32                  & 42.94 $\pm$ 2.63                      & \textbf{0.29} $\pm$\textbf{0.45}  & \textbf{0.06}  &  0.013$\pm$0.021          & 0.0071         \\ \hline
    PCA 64                  & 33.96 $\pm$ 2.01                      & 0.48 $\pm$ 0.53                   & 0.16           &  0.016$\pm$0.024          & 0.0091         \\ \hline
    PCA 128                 &\textbf{27.29} $\pm$\textbf{1.87}      & 0.65 $\pm$ 0.54                   & 0.62           &  0.025$\pm$0.033          & 0.013          \\ \hline
    NN 32                   & 59.65 $\pm$ 2.78                      & 0.093 $\pm$ 0.11                  & 0.07           &  0.010$\pm$0.014          & 0.0068         \\ \hline
    NN 64                   & 49.52 $\pm$ 2.19                      &\textbf{0.083} $\pm$\textbf{0.10}  & 0.06           & \textbf{0.0097}$\pm$\textbf{0.012}          & \textbf{0.0066}         \\ \hline
    NN 128                  & 46.19 $\pm$ 2.23                      & 0.087 $\pm$ 0.12                  &\textbf{0.05}   & 0.0099$\pm$0.012          & 0.0065         \\ \hline
    Parallel PCA 64+NN 64   & 33.63 $\pm$ 1.98                      & 0.27 $\pm$ 0.39                   & 0.07           & 0.014 $\pm$0.021          & 0.0071         \\ \hline
    Sequential PCA 64+NN 64 & 33.95 $\pm$ 2.01                      & 0.49 $\pm$ 0.56                   & 0.16           & 0.016 $\pm$0.023          & 0.0092         \\ \hline
    Gaussian Blur 9x9x9     &  -                                    & \textbf{0.05}$\pm$\textbf{0.04}   &\textbf{0.04}   & \textbf{0.0077}$\pm$\textbf{0.0083}         & \textbf{0.0052}         \\ \hline
    \end{tabular}
    \caption {Average results across all datasets}
    \end{centering}
\end{table*}

